Optimal Transport-Induced Samples against Out-of-Distribution Overconfidence

Deep neural networks (DNNs) often produce overconfident predictions on out-of-distribution (OOD) inputs, undermining their reliability in open-world environments. Singularities in semi-discrete optimal transport (OT) mark regions of semantic ambiguity, where classifiers are particularly prone to unwarranted high-confidence predictions. Motivated by this observation, we propose a principled framework to mitigate OOD overconfidence by leveraging the geometry of OT-induced singular boundaries. Specifically, we formulate an OT problem between a continuous base distribution and the latent embeddings of training data, and identify the resulting singular boundaries. By sampling near these boundaries, we construct a class of OOD inputs, termed optimal transport-induced OOD samples (OTIS), which are geometrically grounded and inherently semantically ambiguous. During training, a confidence suppression loss is applied to OTIS to guide the model toward more calibrated predictions in structurally uncertain regions. Extensive experiments show that our method significantly alleviates OOD overconfidence and outperforms state-of-the-art methods.

==> 8-Rebuttal.tex <==
% \section{rebuttal-appenendix}

% \begin{wraptable}[8]{r}{0.6\textwidth}
%     \vspace{-8mm}
%     \centering
%     \caption{Expected Calibration Error (ECE, $\times 10^{-2}$, ↓) on in-distribution (ID) Datasets for all methods.}
%     \label{tab:ece-id}
%     \setlength{\tabcolsep}{1.0mm}
%     \scalebox{0.75}{
%     \begin{tabular}{c|ccccccc|cc}
%     \Xhline{1.0px}
%     Dataset   & Base          & CEDA          & ACET & CCUs  & CODEs & VOS  & Ours          & OE            & CCUd \\  \hline
%     CIFAR-10  & 3.77          & 4.61          & 3.73 & 3.81  & 4.26  & 2.95 & \textbf{1.88} & 3.65          & 2.91 \\
%     CIFAR-100 & \textbf{6.08} & 11.34         & 9.70 & 12.88 & 11.45 & 8.97 & 6.91          & 9.69          & 6.16 \\
%     SVHN      & 2.10          & 1.83          & 1.30 & 2.82  & 2.74  & 1.51 & 1.66          & \textbf{1.28} & 1.67 \\
%     MNIST     & 0.21          & \textbf{0.14} & 0.16 & 0.37  & 0.31  & 0.24 & \textbf{0.14} & 0.34          & 0.30 \\
%     FMNIST    & 4.00          & 3.61          & 4.12 & 4.53  & 4.65  & 3.39 & \textbf{3.26} & 4.50          & 3.32 \\
%     ImageNet  & \textbf{2.05} & 3.07          & 2.64 &  -    & 4.75  & 4.26 & 2.71          &   -           &  -   \\ 
%     \Xhline{1.0px}
%     \end{tabular}}
%     \vspace{-3mm}
% \end{wraptable}
% \textbf{ID calibration on in-distribution data.} 
% Table~\ref{tab:ece-id} reports the Expected Calibration Error (ECE) of all methods on ID test sets. Across datasets, OTIS does not degrade calibration on correctly classified ID samples and often improves it compared to both the base classifier and OOD-training baselines. On CIFAR-10 and FMNIST, OTIS attains the lowest ECE among all methods (1.88 and 3.26, respectively), and on MNIST it matches CEDA for the best result. On the more challenging CIFAR-100 and ImageNet datasets, several OOD-based methods (CEDA, ACET, CCUs, CODEs) substantially increase ECE relative to the base model, whereas OTIS remains close to the baseline (6.91 vs.\ 6.08 on CIFAR-100, 2.71 vs.\ 2.05 on ImageNet). These results indicate that OTIS does not mitigate overconfidence on OOD inputs by simply making the classifier less confident on ID data; instead, it preserves, and sometimes improves, ID calibration while reducing overconfidence on OOD samples.


% \begin{wraptable}[11]{r}{0.6\textwidth}
%     \vspace{-7mm}
%     \centering
%     \caption{
%     Comparison of different methods on CIFAR-10-C and CIFAR-100-C corruption benchmarks.
%     }
%     \label{tab:corruption}
%     % \setlength{\tabcolsep}{2.0pt}
%     \scalebox{0.75}{
%     \begin{tabular}{c|ccc|ccc}
%     \Xhline{1.0px}
%     \multirow{2}{*}{Method} &
%     \multicolumn{3}{c|}{CIFAR-10-C} &
%     \multicolumn{3}{c}{CIFAR-100-C} \\ \cline{2-7}
%     & MMC$\downarrow$ & FPR95$\downarrow$ & AUROC$\uparrow$
%     & MMC$\downarrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ \\ \hline
%     Base   & 93.21 & 83.30 & 70.43 & 65.61 & 84.06 & 68.92 \\
%     CEDA   & 86.81 & 80.92 & 70.66 & 69.85 & 89.30 & 63.17 \\
%     ACET   & 90.81 & 85.00 & 66.16 & 71.80 & 87.40 & 65.62 \\
%     CCUs   & 85.42 & 80.96 & 66.16 & 66.19 & 79.78 & 65.94 \\
%     CODES  & 84.44 & 84.80 & 68.00 & 74.96 & 85.80 & 67.04 \\
%     VOS    & 90.89 & 82.38 & 66.07 & 70.90 & 84.72 & 67.67 \\
%     Ours   & \textbf{70.78} & \textbf{66.16} & \textbf{76.63}
%            & \textbf{59.22} & \textbf{73.82} & 72.72 \\ \hline
%     OE     & 87.75 & 79.86 & 70.15 & 71.18 & 85.20 & 66.16 \\
%     CCUd   & 83.82 & 68.79 & 73.99 & 63.27 & 78.16 & \textbf{79.20} \\
%     \Xhline{1.0px}
%     \end{tabular}}
%     \vspace{-3mm}
% \end{wraptable}
% \textbf{Robustness under common corruptions.}
% Table~\ref{tab:corruption} reports performance on the CIFAR-10-C and CIFAR-100-C corruption benchmarks. On CIFAR-10-C, OTIS reduces MMC from 93.21 for the base model to 70.78 and achieves the best FPR95 and AUROC with 66.16 and 76.63. On CIFAR-100-C, OTIS attains the lowest MMC of 59.22 and the best FPR95 of 73.82, while its AUROC of 72.72 remains competitive with the strongest baseline CCUd, which reaches 79.20. These results indicate that OTIS mitigates overconfidence and improves OOD detection under a broad range of common corruptions.




% \begin{wraptable}[12]{r}{0.4\textwidth}
% \vspace{-8mm}
% \centering
% \caption{FID w.r.t.\ CIFAR-10 and mean maximum confidence (MMC, \%) 
% for CIFAR-10 and auxiliary boundary samples used by different OOD-overconfidence mitigation methods.
% }
% \scalebox{0.85}{
% \label{tab:fid_mmc}
% % \setlength{\tabcolsep}{7.0pt}
% \begin{tabular}{ccc}
% \Xhline{1.0px}
% Dataset   & FID   & MMC    \\ \hline
% CIFAR-10  & 0.00  & 97.98  \\ \hline
% % SVHN      & 5.47  & 84.22  \\
% CEDA   & 7.25  & 87.39  \\
% ACET      & 7.49  & \textbf{99.98}  \\
% CODES     & 3.18  & 88.84  \\
% OE        & 5.73  & 84.70  \\
% OTIS      & \textbf{2.45}  & 91.29  \\
% \Xhline{1.0px}
% \end{tabular}}
% \end{wraptable}
% \textbf{Comparison with auxiliary boundary samples.}
% Table~\ref{tab:fid_mmc} reports FID w.r.t.\ CIFAR-10 and mean maximum confidence (MMC) under a CIFAR-10 ResNet-18 baseline for CIFAR-10 itself and for the auxiliary boundary samples used by CEDA, ACET, CODES, OE/CCUd, and OTIS. Among these auxiliary sets, OTIS achieves the smallest FID while still inducing high MMC, meaning that OTIS samples stay closest to the CIFAR-10 distribution and are predicted with high confidence. In contrast, other auxiliary datasets either lie further away from CIFAR-10 (larger FID) or already yield much lower confidence. This indicates that OTIS focuses on near-distribution, high-confidence regions that previous auxiliary schemes under-cover, clarifying the benefit of our OT-based construction over simpler boundary-sample generation methods.



% \begin{wraptable}[9]{r}{0.3\textwidth}
% \vspace{-8mm}
% \centering
% \caption{
% FID to CIFAR-10 features and mean maximum confidence (MMC, \%) for CIFAR-10 and auxiliary data used by different OOD-training methods.
% }
% \label{tab:fid_mmc}
% \scalebox{0.88}{
% \begin{tabular}{ccc}
% \Xhline{1.0px}
% Dataset   & FID   & MMC    \\ \hline
% CIFAR-10  & 0.00  & 97.98  \\ \hline
% CEDA      & 7.25  & 87.39  \\
% ACET      & 7.49  & \textbf{99.98}  \\
% CODES     & 3.18  & 88.84  \\
% OE        & 5.73  & 84.70  \\
% OTIS      & \textbf{2.45}  & 91.29  \\
% \Xhline{1.0px}
% \end{tabular}}
% \end{wraptable}

% \textbf{Near-distribution high-confidence behavior of OTIS.}
% Table~\ref{tab:fid_mmc} reports FID to CIFAR-10 features and mean maximum confidence (MMC) for CIFAR-10 and the auxiliary data used by several OOD-training methods under a ResNet-18 baseline. Among these auxiliary sets, OTIS attains the lowest FID, indicating that OTIS samples stay closest to the CIFAR-10 feature distribution, while still inducing high MMC comparable to in-distribution data. In contrast, other auxiliary datasets either lie further away in feature space or elicit lower confidence. This suggests that OTIS focuses on near-distribution, high-confidence regions that are under-represented in standard training, which explains why OTIS is particularly effective at mitigating OOD overconfidence.

% % \newpage

% % \begin{table}[!t]
% \begin{wrapfigure}[26]{r}{0.6\textwidth}
% \centering
% \vspace{-3mm}
% \caption{
% Ablation of OTIS on CIFAR-10 with different base distributions and autoencoder depths, reporting CIFAR-10 TE, ECE ($\times 10^{-2}$), ID MMC, and OOD MMC, FPR95, and AUROC (all in \%).
% Arrows indicate whether lower or higher values are better.
% }
% \label{tab:distribution}
% % \setlength{\tabcolsep}{1.3mm}{
% % \vspace{-2mm}
% \scalebox{0.68}{
% \begin{tabular}{c|c|cccc}
% \Xhline{1.0px}
% Metric                         & Datasets     & Gaussian        & Shallow         & Deep            & Uniform(Ours)   \\ \hline
% TE$\downarrow$                 & CIFAR-10     & \textbf{7.31}   & 7.60            & 8.55            & 7.52            \\ \hline
% ECE ($\times 10^{-2}$)$\downarrow$ & CIFAR-10     & 2.70            & 2.45            & 2.55            & \textbf{1.88}   \\ \hline
% ID MMC$\uparrow$               & CIFAR-10     & \textbf{96.48}  & 96.00           & 92.31           & 95.46           \\ \hline
% \multirow{9}{*}{OOD MMC$\downarrow$} & SVHN         & 17.77           & 24.95           & 14.27           & \textbf{13.18}  \\
%                                  & CIFAR-100    & 68.81           & 67.74           & \textbf{59.83}  & 64.79           \\
%                                  & LSUN\_CR     & 39.33           & 34.47           & 34.72           & \textbf{30.36}  \\
%                                  & Textures\_C  & 57.77           & 56.88           & 54.57           & \textbf{48.75}  \\
%                                  & Noise        & 24.23           & 28.70           & 21.59           & \textbf{16.18}  \\
%                                  & Uniform      & \textbf{10.00}  & \textbf{10.00}  & 10.04           & \textbf{10.00}  \\
%                                  & Adv. Noise   & 27.91           & 44.51           & 31.37           & \textbf{26.42}  \\
%                                  & Adv. Samples & 59.96           & 60.21           & 59.63           & \textbf{57.71}  \\
%                                  & CIFAR-10-C   & 75.07           & 73.85           & \textbf{64.97}  & 70.78           \\ \hline
% \multirow{9}{*}{FPR95$\downarrow$}   & SVHN         & 1.54            & 3.11            & 1.23            & \textbf{1.21}   \\
%                                  & CIFAR-100    & 64.78           & 65.34           & 68.63           & \textbf{63.38}  \\
%                                  & LSUN\_CR     & 15.83           & 19.27           & 22.77           & \textbf{10.95}  \\
%                                  & Textures\_C  & 45.64           & 46.22           & 50.07           & \textbf{36.70}  \\
%                                  & Noise        & \textbf{0.00}   & 0.23            & 4.54            & \textbf{0.00}   \\
%                                  & Uniform      & \textbf{0.00}   & \textbf{0.00}   & \textbf{0.00}   & \textbf{0.00}   \\
%                                  & Adv. Noise   & 3.43            & 3.00            & 1.09            & \textbf{0.66}   \\
%                                  & Adv. Samples & 76.78           & 77.55           & 78.64           & \textbf{74.71}  \\
%                                  & CIFAR-10-C   & 69.04           & 68.60           & 66.96           & \textbf{66.16}  \\ \hline
% \multirow{9}{*}{AUROC$\uparrow$}     & SVHN         & 99.71           & 99.27           & 99.50           & \textbf{99.79}  \\
%                                  & CIFAR-100    & \textbf{87.25}  & 86.78           & 84.91           & 87.19           \\
%                                  & LSUN\_CR     & 97.61           & 97.07           & 96.02           & \textbf{98.26}  \\
%                                  & Textures\_C  & 91.50           & 91.42           & 91.38           & \textbf{93.01}  \\
%                                  & Noise        & 99.78           & 99.48           & 97.26           & \textbf{99.97}  \\
%                                  & Uniform      & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} \\
%                                  & Adv. Noise   & 93.83           & 91.96           & 92.07           & \textbf{95.78}  \\
%                                  & Adv. Samples & 63.37           & 60.97           & 64.47           & \textbf{67.27}  \\
%                                  & CIFAR-10-C   & 75.65           & 75.87           & 75.46           & \textbf{76.63}  \\
% \Xhline{1.0px}
% \end{tabular}}
% % }
% % \vspace{-2mm}
% \end{wrapfigure}
% % \end{table}


% \textbf{Robustness to base distribution and autoencoder depth.}
% Table~\ref{tab:distribution} reports an ablation on CIFAR-10 over different base distributions and depths of the encoder–decoder network. The column Gaussian replaces the uniform base with an isotropic Gaussian while keeping the same autoencoder depth as our default model. The columns Shallow and Deep use a shallower three-layer and a deeper seven-layer symmetric encoder–decoder with a uniform base. The column Uniform(Ours) corresponds to the uniform base combined with a five-layer symmetric encoder and a five-layer symmetric decoder, which is the configuration used in the main experiments.

% Across these variants, the CIFAR-10 test error changes only slightly, which shows that OTIS maintains similar in-distribution accuracy. The uniform base with the five-layer symmetric encoder–decoder achieves the lowest ECE of 1.88 while preserving high ID MMC. On out-of-distribution datasets, this configuration typically attains the lowest or near-lowest OOD MMC and FPR95 and the highest AUROC on most benchmarks, including SVHN, LSUN\_CR, Textures\_C, Noise, adversarial noise, and adversarial samples, with only minor differences on CIFAR-10-C. This indicates that OTIS is robust to the choice of base distribution and encoder–decoder depth and supports using the uniform base with the five-layer symmetric autoencoder as the default design in the main experiments.






\if 0
\textbf{Complexity and scalability of the OT solver.}
We thank the rQDu Q3 for pointing out the potential complexity issues of solving a semi-discrete OT problem on large datasets. In our implementation, the OT problem is solved once on the \emph{full} training set in the latent feature space, rather than on mini-batches of target points. Let $N$ be the number of training examples, $d$ the latent dimension, and $K$ the number of OT cells. Evaluating the dual objective and the associated Laguerre diagram scales as $O(NK)$ in time and $O(N(d+K))$ in memory. Because we operate in a compressed latent space instead of the input space, this significantly reduces the effective dimensionality and memory usage. Concretely, for CIFAR-10 (32$\times$32 inputs, $N=50\mathrm{k}$, latent dimension 256), the OT stage uses about $305.6$ MB of GPU memory, and for ImageNet-resolution features (224$\times$224 inputs with latent dimension 1024) the maximum GPU memory usage is about $12.5$ GB. Both configurations comfortably fit on a 24 GB GPU, demonstrating that the OT computation is practically feasible on the full CIFAR-10 and ImageNet training sets.

Importantly, all reported results are obtained from a \emph{global} semi-discrete OT solution on the full training set, without any mini-batch approximation of the Laguerre cells, so there is no batch-to-batch instability in the geometric partition. We agree, however, that for substantially larger datasets or higher-dimensional latent spaces it would be natural to combine our formulation with mini-batch or distributed OT solvers to further reduce runtime and memory, and to study theoretical guarantees on the quality of the resulting approximate partition (e.g., in terms of Hausdorff distance to the exact Laguerre diagram). We view this as an interesting direction for future work inspired by the reviewer’s suggestion.

\textbf{On Eq.~(11) and the weighting scheme.}
We thank the mC83 Q2 for pointing out this discrepancy. In an earlier prototype
we indeed used a fixed coefficient $0.5$ to combine the two terms, and the line
the reviewer refers to comes from that debugging version. In the current method
and experiments we follow Eq.~(11) and use the inverse-distance weights $A$, which
we found to be slightly more principled while behaving similarly in practice.
We apologize for the inconsistent notation and will clean up the released code
and update the text to clearly reflect the final inverse-distance formulation.

% \textbf{mC83 Q5: Adversarial Noise/Samples in Table 3.}
% We apologize for not fully specifying the attack details. For both “Adversarial Noise’’ and “Adversarial Samples’’ in Table~3 we use a standard $\ell_\infty$ PGD attack. The perturbation budget is $\varepsilon = 8/255$, with 10 gradient steps and a step size of $2/255$, initialized from a random point inside the $\ell_\infty$ ball. “Adversarial Samples’’ are generated from clean CIFAR-10 images by maximizing the cross-entropy loss with respect to the true label. “Adversarial Noise’’ starts from random noise images and optimizes the same loss so that the model assigns a high-confidence prediction to each noise input. The same attack configuration is used for all methods, including VOS and OTIS, so the reported numbers are directly comparable.

% The large gap between VOS and OTIS on adversarial noise is consistent with the design goals of the two methods. VOS synthesizes virtual outliers from low-likelihood regions of the class-conditional feature distributions and mainly regularizes the decision boundary near the in-distribution manifold. It is not explicitly trained against worst case, gradient aligned perturbations starting from random noise, which can lead to high MSP confidence and high FPR95 on our adversarial noise benchmark. In contrast, OTIS constructs singular points that lie close to the classifier’s decision boundaries in the latent space and explicitly pushes the model to assign low confidence in these high risk regions. This makes OTIS particularly effective on “hard’’ near boundary OOD such as adversarial noise and adversarial examples, which explains the striking improvement in FPR95 in Table~3 while still maintaining strong ID accuracy and calibration.
\textbf{On the generation of Adversarial Noise/Samples and the large FPR95 gap.}
We apologize for not fully specifying the attack details. Following the CCUd implementation, both “Adversarial Noise’’ and “Adversarial Samples’’ in Table~3 are generated by an iterative $\ell_\infty$ attack with perturbation budget $\varepsilon = 0.3$, 200 gradient steps, and an initial step size of $0.001$ (with per-sample step-size backtracking), while clipping inputs to $[0,1]$. “Adversarial Samples’’ are obtained by attacking clean CIFAR-10 images, whereas “Adversarial Noise’’ starts from i.i.d.\ uniform random noise. The same attack configuration is used for all methods (including VOS, CCUd, and ours), so the reported numbers are directly comparable.

The large gap between VOS and OTIS on adversarial noise is consistent with the way the two methods construct their auxiliary data. VOS synthesizes virtual outliers from low-likelihood regions of the class-conditional feature distributions and mainly regularizes the decision boundary in the vicinity of the in-distribution manifold, without explicitly targeting worst-case, gradient-aligned perturbations that start from random noise. In contrast, OTIS uses OT to generate singular points in the latent space that lie off the data manifold in low-density, high-risk regions where the classifier is more sensitive. Training the model to assign low confidence on these singular points makes OTIS particularly effective on difficult OOD inputs such as adversarial noise and adversarial examples, which explains the strong improvement in FPR95 reported in Table~3.
\fi
% \textbf{Answer rQDu Q1 and u5rM Q2}
% about KNN

% \begin{table}[!t]
% \centering
% \vspace{-3mm}
% \caption{ECE $(10^{-2})$ ↓}
% \label{tab:mc-imagenet}
% \setlength{\tabcolsep}{1.3mm}{
% % \vspace{-2mm}
% \scalebox{0.9}{
% \begin{tabular}{c|ccccccc|cc}
% \Xhline{1.0px}
% Dataset   & Base          & CEDA          & ACET & CCUs  & CODEs & VOS  & Ours          & OE            & CCUd \\  \hline
% CIFAR-10  & 3.77          & 4.61          & 3.73 & 3.81  & 4.26  & 2.95 & \textbf{1.88} & 3.65          & 2.91 \\
% CIFAR-100 & \textbf{6.08} & 11.34         & 9.70 & 12.88 & 11.45 & 8.97 & 6.91          & 9.69          & 6.16 \\
% SVHN      & 2.10          & 1.83          & 1.30 & 2.82  & 2.74  & 1.51 & 1.66          & \textbf{1.28} & 1.67 \\
% MNIST     & 0.21          & \textbf{0.14} & 0.16 & 0.37  & 0.31  & 0.24 & \textbf{0.14} & 0.34          & 0.30 \\
% FMNIST    & 4.00          & 3.61          & 4.12 & 4.53  & 4.65  & 3.39 & \textbf{3.26} & 4.50          & 3.32 \\
% ImageNet  & \textbf{2.05} & 3.07          & 2.64 &  -    & 4.75  & 4.26 & 2.71          &   -           &  -   \\ 
% \Xhline{1.0px}
% \end{tabular}}}
% \vspace{-2mm}
% \end{table}



% \begin{table}[!t]
% \centering
% \vspace{-3mm}
% \caption{ECE $(10^{-2})$ ↓}
% \label{tab:mc-imagenet}
% \setlength{\tabcolsep}{1.3mm}{
% % \vspace{-2mm}
% \scalebox{0.9}{
% \begin{tabular}{c|ccc|ccc}
% \Xhline{1.0px}
% \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{CIFAR-10-C}                                                  & \multicolumn{3}{c}{CIFAR-100-C}                                                 \\ \cline{2-7}
% \multicolumn{1}{c|}{}                        & \multicolumn{1}{c}{MMC} & \multicolumn{1}{c}{FPR95} & \multicolumn{1}{c|}{AUROC} & \multicolumn{1}{c}{MMC} & \multicolumn{1}{c}{FPR95} & \multicolumn{1}{c}{AUROC} \\ \hline
% Base                                        & 93.21                   & 83.30                     & 70.43                     & 65.61                   & 84.06                     & 68.92                     \\
% CEDA                                        & 86.81                   & 80.92                     & 70.66                     & 69.85                   & 89.30                     & 63.17                     \\
% ACET                                        & 90.81                   & 85.00                     & 66.16                     & 71.80                   & 87.40                     & 65.62                     \\
% CCUs                                        & 85.42                   & 80.96                     & 66.16                     & 66.19                   & 79.78                     & 65.94                     \\
% CODES                                       & 84.44                   & 84.80                     & 68.00                     & 74.96                   & 85.80                     & 67.04                     \\
% VOS                                         & 90.89                   & 82.38                     & 66.07                     & 70.90                   & 84.72                     & 67.67                     \\
% Ours                                        & \textbf{70.78}          & \textbf{66.16}            & \textbf{76.63}            & \textbf{59.22}          & \textbf{73.82}            & 72.72                     \\
% OE                                          & 87.75                   & 79.86                     & 70.15                     & 71.18                   & 85.20                     & 66.16                     \\
% CCUd                                        & 83.82                   & 68.79                     & 73.99                     & 63.27                   & 78.16                     & \textbf{79.20}            \\
% \Xhline{1.0px}
% \end{tabular}}}
% \vspace{-2mm}
% \end{table}


% \begin{figure*}[!t]
% \centering
% \includegraphics[width=1.0\textwidth]{rebuttal_img/rebuttel1.png}
% %\vspace{-3.4mm}
% \caption{
% Histograms of maximum confidence scores on large-scale OOD datasets. A ResNet-50 is trained on ImageNet and evaluated on OpenImage-O, iNaturalist, SUN, and Places.
% }
% %\vspace{-3mm}
% \label{fig:hist_imagenet}
% \end{figure*}



\if 0
rQDu：
1.为什么OT邻域比KNN方法而言是必要的
% 2.ID样本的ECE指标测量
% 3.超大图像数据集构建奇异集的困难（可行性和查找时间）
% 4.CIFAR-10-C上的指标度量
rating:4 conf:4

u5rM:
% 1.动机不明确，为什么要用OT方法，作者没有详细解释为什么OT比其他方法更有效
2.公式6在实验部分说明了（！！！） 公式7的抽取就是我们用KNN寻找夹角的过程
% 3.存在测量误差，对基线方法描述较少
% 4.编码器训练不足的后果是什么
rating:4 conf:3

QHM5:
% 1.测量误差
% 2.157行："these regions often correspond to high-confidence mispredictions" 解释为什么、和神经网络训练过程有没有联系
rating:8 conf:3

mC83:
% 1.公式9角度偏差评分是一种经验支撑，不是定理
% 2.权重λ_i确实不是0.5（公式11）
% 3.基本分布选择对最终结果的高级说明
% 4.ImageNet上的ECE/Brirer/NLL指标去说明ID MMC上升的问题
% 5.CIFAR-10上 FPR95 （vos 94.12%/our 0.66%）差距明显，直观说明下
% 6.编码器的重建质量对结果的影响问题
rating:4 conf:4

\fi

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

